MMICT: Boosting Multi-Modal Fine-Tuning with In-Context Examples

Although In-Context Learning (ICL) brings remarkable performance gains to Large Language Models (LLMs), the improvements remain lower than fine-tuning on downstream tasks. This paper introduces Multi-Modal In-Context Tuning (MMICT), a novel multi-modal fine-tuning paradigm that boosts multi-modal fine-tuning by fully leveraging the promising ICL capability of multi-modal LLMs (MM-LLMs). We propose the Multi-Modal Hub (M-Hub), a unified module that captures various multi-modal features according to different inputs and objectives. Based on M-Hub, MMICT enables MM-LLMs to learn from in-context visual-guided textual features and subsequently generate outputs conditioned on the textual-guided visual features. Moreover, leveraging the flexibility of M-Hub, we design a variety of in-context demonstrations. Extensive experiments on a diverse range of downstream multi-modal tasks demonstrate that MMICT significantly outperforms traditional fine-tuning strategy and the vanilla ICT method that directly takes the concatenation of all information from different modalities as input. Our implementation is available at: https://github.com/KDEGroup/MMICT.

==> ab_feature.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{The different level of feature extraction on VanillaFT.}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{llcll}
\hline
\multirow{3}{*}{LLM}    & \multirow{3}{*}{Level} & \multicolumn{3}{c}{MSVD}                                                   \\ \cline{3-5} 
                        &                        & \multicolumn{2}{c}{Caption}                  & \multicolumn{1}{c}{VideoQA} \\
                        &                        & B@4                  & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{test}    \\ \hline
\multirow{2}{*}{OPT}    & Frame                  &                      & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{}        \\
                        & Video                  & \multicolumn{1}{l}{} &                       &                             \\ \hline
\multirow{2}{*}{FlanT5} & Frame                  & \multicolumn{1}{l}{} &                       &                             \\
                        & Video                  & \multicolumn{1}{l}{} &                       &                             \\ \hline
\end{tabular}
}
\label{tb:ab_feat}
\end{table}

==> test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}lllllllllll@{}}
\multirow{3}{*}{LLM}    & \multirow{3}{*}{Method}           & \multicolumn{6}{c}{Caption}                                                                                                                         & \multicolumn{1}{c}{VQA}   & \multicolumn{2}{c}{VideoQA}                           \\ \cmidrule(l){3-11} 
                        &                                   & \multicolumn{2}{c}{COCO}                        & \multicolumn{2}{c}{MSRVTT}                      & \multicolumn{2}{c}{MSVD}                        & \multicolumn{1}{c}{VQAv2} & \multicolumn{1}{c}{MSRVTT} & \multicolumn{1}{c}{MSVD} \\ \cmidrule(l){3-11} 
                        &                                   & \multicolumn{1}{c}{B@4} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{B@4} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{B@4} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{val}   & \multicolumn{1}{c}{test}   & \multicolumn{1}{c}{test} \\
\multicolumn{2}{l}{VLAB}                                    &                         &                       &                         &                       &                         &                       &                           &                            &                          \\
\multicolumn{2}{l}{VAST}                                    &                         &                       &                         &                       &                         &                       &                           &                            &                          \\
\multicolumn{2}{l}{mPLUG-2}                                 &                         &                       &                         &                       &                         &                       &                           &                            &                          \\
\multirow{3}{*}{FlanT5} & VanillaFT                         &                         &                       &                         &                       &                         &                       &                           &                            &                          \\
                        & VanillaICL-$\text{B}_{\text{VT}}$ &                         &                       &                         &                       &                         &                       &                           &                            &                          \\
                        & \ours                             &                         &                       &                         &                       &                         &                       &                           &                            &                          \\
\multirow{3}{*}{OPT}    & VanillaFT                         &                         &                       &                         &                       &                         &                       &                           &                            &                          \\
                        & VanillaICL-$\text{B}_{\text{VT}}$ &                         &                       &                         &                       &                         &                       &                           &                            &                          \\
                        & \ours                             &                         &                       &                         &                       &                         &                       &                           &                            &                         
\end{tabular}
\end{table}
